Generating Medical Image Counterfactuals using Causal Explanations

Deep learning models have achieved impressive performance in medical image diagnosis, yet their deployment in clinical settings remains constrained by limited explainability. Counterfactual images provide one means of auditing model behavior by showing how an image would need to change for a classifier to produce a different prediction. Existing approaches typically generate such explanations using auxiliary models, including generative adversarial networks and diffusion models. While often capable of producing visually realistic images, these methods explain one black-box model using another, making it difficult to separate the classifier's decision-making process from the inductive biases of the generator. We propose a novel counterfactual-generation framework that requires no generative model. Instead, counterfactuals are constructed directly from causal evidence extracted from the classifier. The resulting approach is deterministic, requires no additional model training, and enables controllable edits within user-specified regions of interest. Experiments on real-world medical imaging datasets demonstrate that the proposed method successfully changes classifier predictions while remaining closer to the original image than generative baselines, providing a more direct and transparent view of the classifier's decision boundary.

==> skin_plot.tex <==
%\subfigure[]{\includegraphics[width=0.24\textwidth]{monalisa.jpg}}

%TODO insert figure
% \begin{figure}[ht]
% \centering 
% \subfigure[Healthy skin lesion]{\label{subfig:skin_lesion_0}\includegraphics[scale=0.35]{images/ISIC_0000014/original.jpg}}
% \hfill
% \subfigure[Counterfactual with our approach]{\label{subfig:skin_lesion_1}\includegraphics[scale=0.35]{images/ISIC_0000014/se.jpg}}
% \hfill
% \subfigure[Naive lesion patching]{\label{subfig:naive_lesion}\includegraphics[scale=0.35]{images/ISIC_0000014/nps.jpg}}
% \hfill
% \subfigure[GAN output]{\label{subfig:gan_output}\includegraphics[scale=0.35]{images/ISIC_0000014/gan.jpg}}

% \caption{Our approach compared to other techniques. \Cref{subfig:skin_lesion_0} shows a healthy skin lesion. Using our
% method, we generate~\Cref{subfig:skin_lesion_1}. If we apply `naive patching' we get~\Cref{subfig:naive_lesion}. This is
% classified as positive, but most of the original lesion has been replaced. Finally,~\Cref{subfig:gan_output} shows an output using the GAN approach. This is classified as positive, but is not informative to the user.}%
% \label{fig:result_images}

% \end{figure}

% --- Column 1 ---
% \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[scale=0.22]{images/TCGA_CS_6186_20000601_14/original.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.22]{images/TCGA_DU_5851_19950428_26/original.jpg}
%     \caption{Original}
% \end{subfigure}
% \hfill

% % --- Column 2 ---
% \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[scale=0.22]{images/TCGA_CS_6186_20000601_14/ne.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.22]{images/TCGA_DU_5851_19950428_26/ne.jpg}
%     \caption{\CE}
% \end{subfigure}
% \hfill
% % --- Column 3 ---
% \begin{subfigure}[t]{0.16\linewidth}
%     \centering
    
%     \includegraphics[scale=0.22]{images/TCGA_CS_6186_20000601_14/npn.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.22]{images/TCGA_DU_5851_19950428_26/npn.jpg}
%     \caption{\NPC}
% \end{subfigure}
% \hfill
% \begin{subfigure}[t]{0.16\linewidth}
%     \centering
    
%     \includegraphics[scale=0.249]{images/ISIC_0000014/original.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.249]{images/ISIC_0000113/original.jpg}
%     \caption{Original}
% \end{subfigure}
% \hfill
% % --- Column 2 ---
% \begin{subfigure}[t]{0.16\linewidth}
%     \centering
    
%     \includegraphics[scale=0.249]{images/ISIC_0000014/se.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.249]{images/ISIC_0000113/se.jpg}
%     \caption{\CE}
% \end{subfigure}
% \hfill
% % --- Column 3 ---
% \begin{subfigure}[t]{0.16\linewidth}
%     \centering
%     \includegraphics[scale=0.249]{images/ISIC_0000014/nps.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.249]{images/ISIC_0000113/nps.jpg}
%     \caption{\NPC}
% \end{subfigure}

% \caption{Examples for counterfactuals generated using our approach (\CE) and a naive patching approach (\NPC). Simply putting an explanation of another image as a patch could completely change the image if the explanation takes up a large part of the image.}
% \label{fig:brain-images}
% \end{figure}
% with GAN
% \begin{figure}[t]
% \centering

% % --- Column 1 ---
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[scale=0.23]{images/TCGA_CS_6186_20000601_14/original.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/TCGA_DU_5851_19950428_26/original.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000014/original.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000113/original.jpg}
%     \caption{Original}
% \end{subfigure}
% \hfill
% % --- Column 2 ---
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[scale=0.23]{images/TCGA_CS_6186_20000601_14/ne.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/TCGA_DU_5851_19950428_26/ne.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000014/se.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000113/se.jpg}
%     \caption{Our approach}
% \end{subfigure}
% \hfill
% % --- Column 3 ---
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[scale=0.23]{images/TCGA_CS_6186_20000601_14/npn.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/TCGA_DU_5851_19950428_26/npn.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000014/nps.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000113/nps.jpg}
%     \caption{Naive Patching}
% \end{subfigure}
% \hfill
% % --- Column 4 ---
% \begin{subfigure}[t]{0.24\linewidth}
%     \centering
%     \includegraphics[scale=0.23]{images/TCGA_CS_6186_20000601_14/gan.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/TCGA_DU_5851_19950428_26/gan.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000014/gan.jpg}
    
%     \medskip
    
%     \includegraphics[scale=0.23]{images/ISIC_0000113/gan.jpg}
%     \caption{GAN}
% \end{subfigure}

% \caption{...}
% \label{fig:brain-images}
% \end{figure}

